Understanding User Perspectives on Prompts for Brief Reflection on Troubling Emotions

We investigate users' perspectives on an online reflective question activity (RQA) that prompts people to externalize their underlying emotions on a troubling situation. Inspired by principles of cognitive behavioral therapy, our 15-minute activity encourages self-reflection without a human or automated conversational partner. A deployment of our RQA on Amazon Mechanical Turk suggests that people perceive several benefits from our RQA, including structured awareness of their thoughts and problem-solving around managing their emotions. Quantitative evidence from a randomized experiment suggests people find that our RQA makes them feel less worried by their selected situation and worth the minimal time investment. A further two-week technology probe deployment with 11 participants indicates that people see benefits to doing this activity repeatedly, although the activity may get monotonous over time. In summary, this work demonstrates the promise of online reflection activities that carefully leverage principles of psychology in their design.

==> scrap/1-intro-extra.tex <==
% These questions ask people to notice, analyze, and revise thoughts and emotions surrounding stressful situations. Such questions are typically posed within extensive psychoeducation or therapy sessions. Here we explore their use within a brief, isolated activity. People's qualitative responses suggest that RQA may offer benefits along the lines of those found from CBT sessions, including structured awareness of thoughts, re-framing of interpretations, and problem-solving around managing emotions. We find the RQA was as effective for stress reduction and perceived to be as beneficial as receiving information from established mental health resources, and more effective than simply asking people to write about their stressful situation.

% We explore the effects and experiences of a brief online reflective questions activity (RQA), which uses a sequence of nine questions inspired by Cognitive Behavioral Therapy. These questions ask people to notice, analyze, and revise thoughts and emotions surrounding stressful situations. Such questions are typically posed within extensive psychoeducation or therapy sessions. Here we explore their use within a brief, isolated activity. People's qualitative responses suggest that RQA may offer benefits along the lines of those found from CBT sessions, including structured awareness of thoughts, re-framing of interpretations, and problem-solving around managing emotions. We find the RQA was as effective for stress reduction and perceived to be as beneficial as receiving information from established mental health resources, and more effective than simply asking people to write about their stressful situation.

%%%%%%%%%%%%%%%%%%%%%%%
% INTRO


% This paper takes a first step towards exploring people’s responses to a brief online intervention that prompts reflection on thoughts and emotions by typing answers to questions, an intervention we call a reflective questions activity (RQA). This is designed by adapting elements of traditionally in-person CBT activities so they can be delivered in a brief online activity that people can do on their own. In particular, our RQA prompts individuals to identify a specific stressful or troubling situation to articulate the thoughts and feelings underlying that situation, to reflect on why they are troubled, and to consider alternative ways of thinking.

% Such micro-interventions \cite{elefant2017microinterventions} can lead to immediate effects on mood, but they do not provide much insight into what users' perspective and experience are on these activities. In addition, CBT-inspired activities can entail fairly intensive questions, prompting examination of people’s thoughts and feelings surrounding difficult situations. There is surprisingly little data about how people perceive these questions, such as whether they find them useful or worth the additional engagement effort required. People's openness to cognitively demanding reflective questions is especially important to explore, given that the status quo of many online resources is in providing information. 

% This paper takes a first step towards exploring people’s responses to a brief online intervention that prompts people to reflect on their thoughts and emotions by typing answers to questions, an intervention we call a reflective questions activity (RQA). This is designed by trying to adapt elements of CBT-like activities conducted in-person to a brief online activity people can do on their own. In particular, our RQA prompts individuals to identify a specific stressful or troubling situation to articulate the thoughts and feelings underlying that situation, to reflect on why they are troubled, and to consider alternative ways of thinking.


==> scrap/4-study1-extra.tex <==
% Many participants spoke of gaining awareness through reflection as a result of writing about their stressful situation. 
% \begin{quote}
%     \textit{It makes you reflect on your way of thinking. (L2). 
%     “writing them out kind of brings them to the attention of you and kind of shows you exactly what you already know, but in a concrete written way.” (L4). 
%     “makes you think and process and analyse” (M11). 
%     “helped me to put things in perspective while being able to see my thoughts in writing.” (M1).}
% \end{quote}

% Several participants mentioned the activity made them recognise illogical or unhelpful thoughts.
    
% \begin{quote}
%     \textit{ “I would read it and I'm like, ‘oh, that's not a very logical way to deal with my stresses’...yeah I think it's really helpful to have” (L2). 
%     “challenged me to challenge my pattern of thinking” (L5). 
%     “helped me pinpoint my maladaptive coping strategy...led me to think more with my brain and less with my immediate emotional reaction” (M17). }
% \end{quote}
   
% Of the 74 participants in Stage 2, 77\% agreed (21\% slightly, 26\% strongly) with the sentiment that they experienced increased awareness of the situation by reflecting on it.

% \subsubsection{Benefit of Structured Analysis of Situation}
% Another theme arose around the benefits of being able to take a structured approach that helped individuals break down the components of their stressful situation. 
% \begin{quote}
%     \textit{ “it helps you categorize exactly what you were thinking.” (L3). 
%     “the process of having deconstructed it sort of helped me feel calmer about it” (L5). 
%     “awareness through structure helps you put things in the right order” (L2). 
%     “helps you put things in the right order” (M9). 
%     “Thinking through the situation and breaking down my feelings and behavior reduced my dread and anxiety” (M3).}
% \end{quote}

% Of the 74 participants in Stage2, 74\% agreed (23\% slightly. The percentage of participants expressing agreement with “This exercise allowed me to undergo a structured analysis of my situation, which I found helpful” was: Slightly Agree+: 74\%, Agree+: 51\%, Strongly Agree: 13\%.

% \subsubsection{Felt Good to Let Situation out of One's Head}
% Participants mentioned it feeling good to let the thoughts and feelings out of their head and into writing they could see. 

% \begin{quote}
%     \textit{ “helps you get out all your thoughts and feelings and take that weight off of your shoulders.” (L5). “always helpful just to get the thoughts that are piling up out of one's head” (M14). “gets it out of your head and allows you to examine it from an outside perspective” (M11).  “Being able to have someone or something to hear me in the void.” (M2). }
% \end{quote}

% The percentage of participants expressing agreement with “It felt good to write out my situation to let it out of my head” was: Slightly Agree+: 74\%, Agree+: 52\%, Strongly Agree: 20\%.

% \subsubsection{Feelings of Greater Acceptance}

% A theme that came out of online participants’ answers was that the activity helped them gain acceptance of their stress around their issue. 
% \begin{quote}
%     \textit{ “It’s a way to accept some things and admit to issues that I may have” (M6) “Acknowledging stress and accepting it” (M7). }
% \end{quote}

% The percentage of participants expressing agreement with “This activity helped me feel greater acceptance about the stressful situation” was: Slightly Agree+: 70\%, Agree+: 42\%, Strongly Agree: 11\%.

% \subsubsection{Focus on Solutions for Improvement}

% Many participants spoke of the activity as prompting them to adopt a problem solving approach to improve their situation.

% \begin{quote}
%     \textit{ “helped me open up to other possible situations or options” (L3) “I definitely feel like I should work on like finding ways to not make myself in like stressful situation.” (L1). “Instead of panicking into okay what can I do now to fix this situation or to deal with this situation...it makes you think about how you could have handled it differently” (L2). “think it is good helping me process, and realize, and digest what happened and that way I can learn from it” (L5). “helped me focus on solving the problem rather than clinging to it” (M12). “made me think why I feel the way I do and how I am handling it the right way” (M13). }
% \end{quote}

% The percentage of participants expressing agreement with “This activity helped me understand or remember some solutions I could use to improve the situation” was: Slightly Agree+: 72\%, Agree+: 39\%, Strongly Agree: 14\%.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Frustration over Lack of Solution}

% On the other hand, some participants mentioned that the activities did not provide them a solution.
% \begin{quote}
%     \textit{ “it's not like it was like, "oh you know this fixed everything and everything's great now." You know?” (L6). “I realize that changing one's thinking can be helpful in dealing with a problem, but a few questions aren't going to solve or make a situation go away regardless” (M18). “They just made me think about how much pain I was in and really didn't offer any solution whatsoever to the stress” (M19).  }
% \end{quote}

% The percentage of participants expressing agreement with “I felt frustrated/discouraged because this exercise did not help me see solutions to my situation” was: Slightly Agree+: 36\%, Agree+: 19\%, Strongly Agree: 5\%.

% \subsubsection{Unpleasant to Describe the Situation}

% A prevalent negative theme mentioned by many participants was that it was an unpleasant experience to revisit their stressful situation. 

% \begin{quote}
%     \textit{ “I was sort of blaming myself for not having dealt with stuff better” (L5) “Frustration and probably some anxiety.” (L6). “At first I resented being asked to think about something I would like to forget” (M10). “made it worse because now I’m thinking about it again” (M17). “temporarily raised my stress level as it made me think back to this situation because it put me back in the stressful situation and brought back memories and feelings” (M16). “It increased (stress), because I hate writing and reliving the pain I had before” (M4). “I didn't like thinking about this event once again” (M20). }
% \end{quote}

% The percentage of participants expressing agreement with “Having to remember my stressful moment was unpleasant” was: Slightly Agree+: 66\%, Agree+: 39\%, Strongly Agree: 22\%.

% \subsubsection{Trying to Understand Situation Brought Confusion}

% Some participants felt confusion while engaging with the activity.

% \begin{quote}
%     \textit{“I tend to lose track of sort of where I was going with my thoughts sometimes” (L5) “you might be stressed and like that makes sense you, but is it justified? Not really. And it's a weird line to walk. I think” (L3). “I feel confused now by all of these questions” (M20). }
% \end{quote}

% The percentage of participants expressing agreement with “Trying to understand my situation brought more confusion” was: Slightly Agree+: 38\%, Agree+: 23\%, Strongly Agree: 11\%.

%%%%%%%%%%%%%%%%%%%%%%%

% Table~\ref{tab:study1} shows the themes that emerged from the first round of participants and the degree of agreement the second round of participants expressed with them. 
% First and foremost, people appreciated the fact that the RQA provided them with a structured outlet through which they could express their thoughts and feelings.
% Of course, people's thoughts and feelings did not completely disappear after they used the RQA, but were rather transferred into writing that people could reference later.
% As L4 noted,
% \italquote{writing [my thoughts] out kind of brings them to the attention of you and kind of shows you exactly what you already know, but in a concrete written way.}
% Participants referenced the structuring of their thoughts in many ways: ``categorization'' (L3), ``deconstruction'' (L5), ``right order'' (M9), and ``breaking down'' (M3).
% By seeing their thoughts in words, individuals were able to recognize illogical or unhelpful thoughts.
% For example, M17 commented that the RQA ``helped me pinpoint my maladaptive coping strategy...led me to think more with my brain and less with my immediate emotional reaction''.
% Seeing their feelings in front of them also helped participants acknowledge and accept their stress.
% Many participants even acknowledged that the RQA prompted them to adopt a problem-solving approach to improve their situation.
% L2 noted that
% \italquote{Instead of panicking into `okay what can I do now to fix this situation or to deal with this situation', it makes you think about how you could have handled it differently}

% Of course, our RQA was not without its own flaws.
% Some participants mentioned that it was an unpleasant experience to revisit their stressful situation.
% For many, the discomfort was temporary since they had to recollect the details of their situation before they could talk through their feelings and come to a resolution.
% For others, however, the stress lasted longer.
% This was particularly true for participants who decided to go through the RQA using a past stressful situation that was not necessarily affecting them at the current time.
% We recognize that this is a side-effect of the fact that participants were prompted to go through the RQA when they were recruited rather than when they needed to reflect the most.
% Some participants also experienced confusion while engaging with the activity, becoming wrapped in their thoughts and losing track of their line of reasoning.
% Lastly, some participants were frustrated that the RQA did not offer a potential concrete solution to their issues.
% M18 commented,
% \italquote{I realize that changing one's thinking can be helpful in dealing with a problem, but a few questions aren't going to solve or make a situation go away regardless}
% Some participants even felt that the RQA highlighted the pain they were experiencing and ``really didn't offer any solution whatsoever to the stress'' (M19).
% Although more people found the RQA to be a constructive and positive experience than not, these comments highlight the challenges and opportunities in deploying a brief digital intervention for independent reflection.
% Providing suggestions of concrete actions that people could take and encouraging remarks between questions are just some potential directions that designers and researchers can explore for creating a safe and beneficial outlet for people's emotions.
% For the sake of avoiding confounds in our results, however, we continued using the same RQA for our second study.

==> scrap/5-study2-extra.tex <==
% Lastly, almost 79\% of the participants expressed some degree of interest in using the \textit{RQA} in the future.
% A similar fraction of individuals agreed (slightly agreed or stronger) with the statement that the \textit{RQA} was helpful to them in reflecting on or managing their troubling situation.
% Appreciation for the \textit{RQA} was not only reflected in the subjective ratings of the participants, but also their objective behaviors.
% Over 25\% of participants provided their email in order to receive a link to the activity, and over 10\% provided a friend's email to have a link sent to them as well. 
% It should be noted that some people retrieved value in just using the \textit{Explain Situation} prompt, with roughly 57\% of people stating that they would use it in the future and 20\% of people asking to receive the prompt in their email.

% When asked how much they agree with the statement "I would like to use this activity again in the future", participants' average rating of 1.2 sits just above 1 for "Slightly Agree", and reflects that 79\% of participants reported they Slightly Agree+ (Slightly Agree, Agree, and Strongly Agree), 50\% of participants said they Agree+ (Agree, Strongly Agree), and 29\% of participants said they Strongly Agree. These subjective statements corresponded to objective behavior, where over 25\% of participants provided their email in order to receive a link to the activity, and over 10\% provided a friend's email to have a link sent to them as well. 

% When asked to rate the statement ``This was helpful to me in reflecting on and managing my troubling situation.",  79\% of participants said they Slightly Agree+, 57\% of participants said they Agree+, and 31\% of participants said they Strongly Agree.
% Despite the fact that the the RQA took longer than the Explicit Explain Situation  (mean of 8.9 vs 1.6 minutes, as shown in Table 1), there was no significant difference in the mean response of ``Neutral" to the statement ``The activity was too long". This might be because people saw value in the additional time spent.

% \subsubsection{The RQA was more positively received than the Explain Situation condition}

% We aimed to investigate whether the full RQA with 8 follow-up questions was perceived as more beneficial than the Explain Situation prompt alone. One possibility could have been that the extra time and effort for these additional questions was unnecessary, and that the primary value in the activity simply comes from writing anything at all about a troubling situation, given the wide range of research on the benefits of writing and journaling [37]. Another possibility was that additional questions in the the RQA would be overwhelming and the extra effort required would not be perceived as worthwhile.

% People who used the \textit{RQA} reported significantly greater reduction in the extent to which they were troubled by their situation (t(205) = 4.12, p < 0.001). 
% In fact, the \textit{Explain Situation} condition led to an increase in reported stress (t(98) = 2.05, p < 0.05), suggesting that the additional questions from the RQA were necessary to counteract an initial increase in stress from revisiting the situation. 
% This finding highlights a design tradeoff---reflection activities should be brief to be convenient, but not too brief or else people might undermine their faith about such activities in general. 
% Q9 measured people's change in the extent to which they agreed that they could ``Better Manage Stress with the Right Activities and Questions". 
% Our RQA led to significantly greater increase in agreement (a positive trend) than Explain Situation, for which there was a negative trend in the belief that the right activities would help manage stress (a negative trend), (t(195) = 2.06, p < 0.05). 

==> scrap/7-discussion-extra.tex <==
\subsection{The RQA's benefits relative to alternatives} 
The impact of the RQA was not due to merely a placebo effect of giving people an activity, or to the mere action of typing about the situation. Study 2's randomized experiment compared the RQA to an \textit{Explain Situation} control condition that just asked people to type about the situation in a free-form way; this was just the first question in the RQA without the additional questions about thoughts and emotions. The \textit{Explain Situation} condition was significantly less effective and may even have increased how troubled people felt about the situation. This was surprising, as we anticipated that the \textit{Explain Situation} condition could have been equally effective or \textit{more} effective than the RQA because the extended series of questions in the latter could have been confusing, overwhelming, or distracting.
% , while a simpler prompt to explain could have allowed to guide themselves in whatever externalized reflection is most useful.
Although we received qualitative feedback to these effects in Study 1, our results in both studies suggest that participants generally perceive value in the sequence of reflection prompts targeting thoughts and emotions.
By leveraging principles from CBT, the overhead introduced by the new questions was generally outweighted by their benefits. 

\subsection{Challenges for future RQAs.} 
A central consideration for future reflection activities is the understanding that they may cause unpleasant feelings and even potentially trigger negative states. This was most clear for participants in the \textit{Explain Situation} condition who did not engage in any follow-up questioning or information. In the qualitative feedback to this condition, participants spoke of negative feelings and dissatisfaction of the activity ending abruptly without any guidance. The two clinical psychologists in our study highlighted this as a challenge that also arises in CBT and psychotherapy sessions. If someone’s situation or individual characteristics does not respond well to structured analysis, it may be helpful to offer them alternative activities (e.g., meditation) or simply offering a list of potential strategies. Furthermore, It may be prudent to warn users ahead of time that they will be asked to describe a stressful situation, which may cause unpleasant emotions and memories to arise. 

\subsection{Sustaining Benefits Outside of Our RQA} 
Since RQAs can be brief, self-delivered, and immediately useful, they could be valuable in habit formation around the use of evidence-based interventions \cite{eyal_2019}. 
The time needed to gain benefits from CBT therapy or online courses may demotivate users from using them. 
Hence, it is important that users realize the potential benefits they can receive if they make an initial effort to engage with an intervention. 
It is equally important to reinforce engagement with continued support.
One broader opportunity is that RQAs might engage users in seeking out more involved resources for managing emotional well-being. Since online reflection activities are low-cost, scalable, and easily deliverable resources, people who are not seeking treatment may leverage these exercises as a precursor to learning other skills for stress management. Reflective activities could also serve as a gateway to a broader ecosystem of wellbeing reminders and resources. 
For example, a digital intervention could push timely messages related to wellbeing based on an individual’s stress level \cite{paredes2014poptherapy, elefant2017microinterventions}. 
Such stress information could be recorded through periodic ecological momentary assessments or by wearables that estimate stress via physiological signals like heart rate and galvanic skin response (e.g., Fitbit Sense).

\subsection{Improving Our RQA} 
There are also many improvements that could be made in promoting online reflection, particularly in the questions that are included and how users interact with them. Participants pointed out a few cases where questions could be clarified and changed. For example, the question ``Does the trigger truly justify the thought?" was interpreted as a challenge to some individuals. Other participants reported that frustration in the fact that our RQA did not offer concrete solutions. Some participants felt at a loss when asked to think of alternative perspectives on a situation or thought. 
One possibility for future work would be to create a handful of examples for each question that guide users in articulating thoughts, feelings, and alternative framings. As an online intervention, rich multimedia like animations and videos could help in this regard. Another possibility would be to allow users who appreciated the RQA to voluntarily allow their anonymised situation to be put into a tagged database of examples. An information retrieval system can rank the relevance of these examples for any new situation as a constant source of fresh inspiration. With the integration of machine learning algorithms like collaborative filtering algorithms \cite{schafer2007collaborative}, a digital intervention system can suggest closely matched situations that might seem relevant to the user. 
More broadly, there are many opportunities for personalizing reflective questions, example responses, and other features of the online interaction. For example, an RQA can add questions that relieve, remove questions that induce stress, or display previous activity responses as a point of comparison. RQAs can also be combined with other resources and activities, but determining when and how that information should be provided remains an interesting design question.

\subsection{Deployment of RQA via Different Technology}
Study 3 allowed us to to gather important insights about the role of different technology in deploying similar RQAs. We noticed that participants generally favored doing the activity in a big computer screen that allows convenience in typing and editing. At the same time, many of them felt that typical mobile phones are not suited for this sort of interaction. However, it is important to consider how such activities can be promoted via mobile phones because of the medium's ubiquity and scalability \cite{barnes2019mobile}.
When an individual starts writing multi-sentence responses, the text entry box often gets larger and takes up space for prior questions, forcing people to stop writing and scroll up to review past answers \cite{nouri2019assessing}. Moreover, keyboard in a touchscreen mobile phone allows much less flexibility in selecting, copy-pasting, or removing a long text. 

A dedicated mobile application with customized typing features may solve many of these problems. The app can also store 
However, the worldwide growth of mobile mental health systems speak otherwise \cite{inal2020usability}. 
We also noticed that some participants were distracted by the notifications of mobile phones when they were doing the activity, and they felt they have greater control over distracting notifications in computers. This again ask
However, motivating people to install an application also takes significant effort, particularly in the initial stages when users may not have clear about the benefits of doing the RQA. One possible solution in this context could be use of text messages in the 

==> scrap/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> scrap/overview.tex <==
\section{OVERVIEW OF RESEARCH}

\subsection{DESIGN OF ONLINE REFLECTIVE QUESTIONING ACTIVITY (RQA)}

To design our RQA, we first reviewed popular CBT guides meant for personally guided use, including Youper (youper.ai), Depression CBT (\url{https://www.excelatlife.com/apps.htm#depressionapp}), KOKObot (https://www.kik.com/casestudy/koko/) and Woebot (woebot.io) \cite{fitzpatrick2017delivering}. We found that these interventions leverage common CBT techniques such as ``chaining", challenging thought distortions, brainstorming alternatives, and rating mood severity \cite{beck2011cognitive}. Inspired by these guides, we created an RQA to help people reflect: the questions were designed to help them articulate a stressful or troubling situation for reflection, elaborate on the thoughts and emotions elicited by the situation, and consider alternative ways to conceptualize the situation.  The RQA we investigated is shown in Table 2, along with the corresponding CBT techniques upon which each question is based. The RQA starts by asking a person to “think of a particular situation where you felt stressed or had a negative emotion, which you can try to reflect on as you go through this activity. It could be a current situation, one in the past, or one you anticipate in the future." After that, the person is asked to recognize the troubling thoughts, the consequences of those thoughts, and possible alternatives in action or perspective.

To confirm that our RQA was aligned with activities that would be used in psychotherapy, we presented it to four clinical psychologists with expertise in CBT. They verified that our RQA was aligned with existing techniques, but remarked that the questions focused on more advanced techniques that were usually introduced only after several sessions of evaluation and psychoeducation, whether during psychotherapy or as part of homework exercises. They also expressed skepticism that people would know how to respond to the questions or that people would be willing to complete them all in the first place. One clinical psychologist wondered if more than one or two questions might be excessive for an online format with no human-in-the-loop to respond. This motivated our comparison of the RQA with a control condition that simply asked users to explain a troubling situation -- the first question in the RQA. 
